F-coref: Fast, Accurate and Easy to Use Coreference Resolution

We introduce fastcoref, a python package for fast, accurate, and easy-to-use English coreference resolution. The package is pip-installable, and allows two modes: an accurate mode based on the LingMess architecture, providing state-of-the-art coreference accuracy, and a substantially faster model, F-coref, which is the focus of this work. F-coref allows to process 2.8K OntoNotes documents in 25 seconds on a V100 GPU (compared to 6 minutes for the LingMess model, and to 12 minutes of the popular AllenNLP coreference model) with only a modest drop in accuracy. The fast speed is achieved through a combination of distillation of a compact model from the LingMess model, and an efficient batching implementation using a technique we call leftover batching. Our code is available at https://github.com/shon-otmazgin/fastcoref

==> 03_method-old.tex <==
\section{\model{}}
The \model{} Library provide clusters indices, clusters as text, and also logits which can be use in down stream tasks.

We begin with a brief tour. Accessing a dataset is done simply by referring to it by a global identity.  

\begin{lstlisting}[language=python,numbers=none]
dataset = load_dataset("boolq")
\end{lstlisting}

\noindent Each dataset has a features schema and  metadata.

\begin{lstlisting}[language=python,numbers=none]
print(dataset.features, dataset.info)
\end{lstlisting}

\noindent Any slice of data points can be accessed directly without loading the 
full dataset into memory.

\begin{lstlisting}[language=python,numbers=none]
dataset["train"][start:end]
\end{lstlisting}

\noindent  Processing can be applied to every data point in a batched and parallel 
   fashion using standard libraries such as NumPy or Torch.

\begin{lstlisting}[language=python,numbers=none]
# Torch function "tokenize" 
tokenized = dataset.map(tokenize, 
                        num_proc=32)
\end{lstlisting}

The final coreference model of the library is fully defined by two building blocks: (a) knowledge distillation for the coreference task, (b) efficient documents batching implementation, and (c) aggressive mention pruning. Together they produce a small, fast and efficient model for coreference resolution.

\subsection{Knowledge distillation} 

In its simplest form, knowledge distillation involves a teacher model, a student model, and a large training dataset. Particularly for coreference, the teacher model we use is a near\footnote{what is near SOTA} SOTA model, \textsc{s2e} model \cite{kirstain-etal-2021-coreference} and \textsc{lingmess} \cite{Otmazgin2022LingMessLI} which is a variant of the \textsc{s2e} model. \arie{not clear from here} Furthermore, to keep Knowledge distillation principles\footnote{smaller and efficent network} our student model design is smaller version of \textsc{s2e} coreference head on top of DistilRoBERTa \citep{Sanh2019DistilBERTAD} encoder. The \textsc{s2e} head is a memory efficient architecture, and currently address the best\footnote{The CorefQA model~\citep{wu-etal-2020-corefqa} achieves a substantially higher score, but requires to run a separate BERT inference for each mention, making it highly impractical. } performance-efficiency trade-off. In addition, on average, DistilRoBERTa is twice as fast as Roberta-base, this is while the other existing models using the \textit{large} variant.

\arie{be more specific refer to the s2e model not coref models in general}Coreference systems typically includes multiple components: (a) mention scorer, (b) pruning the top scoring mentions, and (c) antecedent scorer. It can be challenging to transfer all the knowledge associated with these components from one model to another.\arie{why?} In both models, the exact same mentions must be prune based on their own individual mention scorer. Additionally, the estimated distribution by the antecedent scorer for each mention $q$ should be considered when transferring knowledge in coreference. Most of the mentions have many false antecedent candidates and a few true antecedents, resulting in a long tail distribution where most of the probabilities are near-zero. In this case, learning from such distribution can undermine the effectiveness of knowledge distillation.\arie{this paragraph should be clearer, maybe you can add the formula of the s2e model in the BG and here refer to the formula}

To address that, we implemented two methods to transfer the coreference knowledge from teacher to student model: hard distillation and soft distillation. Hard distillation is a straightforward method, we label each example in the training dataset with the teacher's predicted clusters, then for each possible mention $q$ at the text, the student's learning objective optimizes the sum of probabilities over the true antecedents $\hat{c}$ of $q$:

\begin{equation}
\label{eq:loss}
L(q) = \log \sum_{\hat{c} \in \mathcal{C}(q) \cap \textsc{gold}(q)}P(\hat{c} \mid q)
\end{equation}

where $\textsc{gold}(q)$ is the teacher predicted cluster contains $q$, and considered as true antecedents of $q$. 

Coreference soft distillation is more complex, but can provide a rich signal by learning from the full antecedent distribution. At the soft distillation method, for each document, the teacher model and the student model scores all possible spans in the text. Then, to have the exact same spans in the next step, the teacher forward to the student the top mention indices obtained by the teacher's mention scorer, then both models prune the mentions based on these indices. Finally both teacher and student estimates an antecedents distributions, $T$ and $S$, and the student objective for each span $q$ described at Eq.~\ref{eq:loss} utilizedataset add item huggingface\arie{?}
these two distributions.
\arie{need to elaborate this paragraph. first enumerate all the parameters that need to be learned and how we learn them, what's the loss etc?}

\subsection{Efficient documents batching}


\arie{consider moving to BG or at least part of it.}
Dynamic batching consists of sorting the instances according to their length in order to batch together instances with similar length. This is a general method for efficiently processing inputs of different sizes with a minimal number of padded tokens. In coreference resolution, documents can be long and exceed the usual max length limit of 512 tokens in BERT-like transformers. 


\arie{we need to start by summarizing the key idea before we get into details}
Given a batch of documents $B$x$D$\arie{what's B and D?}, this constraint\arie{which constraint?} obliges us to split each document into $K$ segments of $M$ length, usually the transformer max length limit ($M$=512). Resulting a batch dimension of $B$x$K$x$M$. Using the aforementioned dynamic batching, this will create batches with similar number of segments with real (not padded) tokens. Zoom in to the batch tensor, we can observe that the most padded tokens are in the last segment of each document.\arie{not clear} For example, assuming a batch of 10 documents of 600 tokens, this batching will create a single batch of 10x2x512, while 10 segments will include 424 padded tokens.\arie{I had to compute the diff to understand this sentence, it's not clear. we should say that for each doc, there is one full segment and one segment with only 88 tokens, so we must add 424 padding tokens to run it together. On average there are XX\% of padded tokens in XX data, so we waste a lot of computation time.} 


To reduce the overall number of padded tokens, we split the batch into two batches of: (1) $B$x$(K-1)$x$M$, and (2) $B$x$L$, where $L$ is the leftover tokens in each document, padded to the max leftover tokens document. In the above example, we will get a large batch of 10x1x512 and a small batch of 10x88. Using dynamic batching we can assume that there are almost 0 padding tokens in the first batch and a small amount of padding tokens in the second batch due to the fact that $L << M$ and the documents are in similar lengths. Furthermore, the leftovers method splits each batch into two batches and forces us to have two transformer forward passes instead of one. Our empirical experiments showed that splitting to two batches is more efficient and faster than having a large amount of padding with one batch. \arie{maybe it's better to show the graph already here, but not sure}

\subsection{Mention pruning}


==> 06_related.tex <==
\section{Related work}

Several works were conducted to address efficiency and lightweight model for coreference. \citet{joshi-etal-2020-spanbert} was the last model to construct a vector representation for each span. Since then, \citet{kirstain-etal-2021-coreference} and our recently developed model variant, \textsc{LingMess} \cite{Otmazgin2022LingMessLI}, removes this costly construction and leverage only the tokens at the start and end of a span, in this way, the coreference model becomes more lightweight and consumes significantly less memory. More recently \citet{dobrovolskii-2021-word} introduced a new approach for solving coreference, where instead of considering coreference links between spans, their model scores each pair of words to be co-referring, and then expand words to spans. By that \citet{dobrovolskii-2021-word} reduced the model complexity from $\mathcal{O}(n^4)$ using spans to $\mathcal{O}(n^2)$ while using words. This development in the efficiency of the conference can be seen at section~\ref{sec:results} in our experiments. Even though the coreference complexity was reduced, in comparison to this work, the aforementioned models are still slow and large due to their number of parameters and layers. Furthermore, the released implementations of these models may be difficult to run, they requires preprocessing steps such as tokenization, sentence parsing, and truncation to maximum document length. A common package that eliminates these issues is AllenNLP \cite{Gardner2017AllenNLP}, while they provide an easy API for coreference, they still utilize the large and inefficient model of \citet{joshi-etal-2020-spanbert}. In our work we considered all together, we reduced the model size, improved the efficiency with batching and released an easy API.


